Instance-Adaptive and Geometric-Aware Keypoint Learning for Category-Level 6D Object Pose Estimation

Category-level 6D object pose estimation aims to estimate the rotation, translation and size of unseen instances within specific categories. In this area, dense correspondence-based methods have achieved leading performance. However, they do not explicitly consider the local and global geometric information of different instances, resulting in poor generalization ability to unseen instances with significant shape variations. To deal with this problem, we propose a novel Instance-Adaptive and Geometric-Aware Keypoint Learning method for category-level 6D object pose estimation (AG-Pose), which includes two key designs: (1) The first design is an Instance-Adaptive Keypoint Detection module, which can adaptively detect a set of sparse keypoints for various instances to represent their geometric structures. (2) The second design is a Geometric-Aware Feature Aggregation module, which can efficiently integrate the local and global geometric information into keypoint features. These two modules can work together to establish robust keypoint-level correspondences for unseen instances, thus enhancing the generalization ability of the model.Experimental results on CAMERA25 and REAL275 datasets show that the proposed AG-Pose outperforms state-of-the-art methods by a large margin without category-specific shape priors.

==> cvpr2024/table/camera_per_cat.tex <==
\begin{table}[h]
    \setlength{\tabcolsep}{3pt}
\caption{\textbf{
    Per-category results of AG-propose on CAMERA25.}
    }
\label{tab:CAMERA25_per_cat}
\centering
\begin{tabular}{c|cc|cccc}
    \hline
    category & $IoU_{50}$ & $IoU_{75}$ & $5^{\circ} \, 2 \, \textbf{cm}$  & $5^{\circ} \, 5 \, \textbf{cm}$  & $10^{\circ} \, 2 \, \textbf{cm}$ & $10^{\circ} \, 5 \, \textbf{cm}$ \\ \hline
    bottle   & 93.7  & 91.4  & 80.9 & 96.4 & 82.3 & 99   \\
    bowl     & 96.9  & 96.7  & 98.7 & 99   & 99.7 & 99.8 \\
    camera   & 89.2  & 84.3  & 57   & 60.9 & 73.6 & 81.1 \\
    can      & 92.1  & 92    & 99.7 & 99.8 & 99.7 & 99.9 \\
    laptop   & 97.5  & 90.8  & 76.1 & 85.9 & 80.6 & 92.4 \\
    mug      & 93.6  & 92.7  & 54.5 & 54.6 & 77.1 & 77.3 \\ \hline
    average  & 93.8  & 91.3  & 77.8 & 82.8 & 85.5 & 91.6 \\ \hline
    \end{tabular}
\end{table}

==> cvpr2024/table/housecat6d.tex <==
\begin{table}
\caption{\textbf{
    Quantitative comparisons with state-of-the-art methods on the HouseCat6D dataset.}
    }
\label{tab:HouseCat6D}
\centering
\begin{tabular}{c|c|cc|cccc}
\hline
Method     & $IoU_{25}$         & $IoU_{50}$         \\ \hline
NOCS [33]          & 50.0            & 21.2          \\
GPV-Pose [5]         & 74.9            & 50.7          \\
VI-Net \cite{lin2023vi}          & 80.7            & 56.4          \\
ours           & \textbf{83.2} & \textbf{68.3} \\ \hline
\end{tabular}
\end{table}

==> cvpr2024/table/housecat6d_nocs_err.tex <==
\begin{table}
\begin{minipage}[t]{0.4\linewidth}
\centering
\caption{\fontsize{5}{12}\textbf{Results on HouseCat6D.}}
% \caption{\textbf{HouseCat6D.}}
\vspace{-0.2cm}
\label{tab:HouseCat6D}
\begin{threeparttable}
\resizebox{\linewidth}{!}{
\setlength\tabcolsep{5pt}
\small
\begin{tabular}{c|c|cc|cccc}
    \hline
    Method     & $IoU_{25}$         & $IoU_{50}$         \\ \hline
    NOCS [33]          & 50.0            & 21.2          \\
    GPV-Pose [5]         & 74.9            & 50.7          \\
    VI-Net           & 80.7            & 56.4          \\
    ours           & \textbf{83.2} & \textbf{68.3} \\ \hline
    \end{tabular}
}
\end{threeparttable}
\end{minipage}
\begin{minipage}[t]{0.5\linewidth}
\centering
\caption{\fontsize{5}{12}\textbf{The percentage of valid correspondences.}}
% \caption{\textbf{proportion.}}
\vspace{-0.2cm}
\label{tab:nocs_err}
\begin{threeparttable}
\resizebox{\linewidth}{!}{
\setlength\tabcolsep{5pt}
\small
\begin{tabular}{c|cccc}
    \hline
    Threshold   & \textless{}0.05 & \textless{}0.1 & \textless{}0.2  \\ \hline
    DPDN [17]    & 18.3            & 41.7           & 62.2                   \\
    IST-Net [18] & 22.6            & 46.8           & 63.8                   \\
    ours    & \textbf{29.5}   & \textbf{54.1}  & \textbf{70}     \\ \hline
    \end{tabular}
}
\end{threeparttable}
\end{minipage}
\vspace{-0.20in}
\end{table}


==> cvpr2024/table/nocs_err.tex <==
\begin{table}
\caption{\textbf{
    The proportion of valid correspondences with errors below different thresholds.}
    }
\label{tab:nocs_err}
\centering
    \begin{tabular}{c|cccc}
    \hline
    Threshold   & \textless{}0.05 & \textless{}0.1 & \textless{}0.2  \\ \hline
    DPDN [17]    & 18.3            & 41.7           & 62.2                   \\
    IST-Net [18] & 22.6            & 46.8           & 63.8                   \\
    ours    & \textbf{29.5}   & \textbf{54.1}  & \textbf{70}     \\ \hline
    \end{tabular}
\end{table}

==> cvpr2024/table/per_cat.tex <==
\begin{table*}
\caption{\textbf{
    Per-category results of our method on CAMERA25 and REAL275 datasets.}
    }
\label{tab:per_cat}
\centering
\begin{tabular}{c|cccccc|cccccc}
    \hline
    \multirow{2}{*}{category} & \multicolumn{6}{c|}{CAMERA25}                                  & \multicolumn{6}{c}{REAL275}                                    \\ \cline{2-13} 
                              & $IoU_{50}$ & \multicolumn{1}{c|}{$IoU_{75}$} & $5^{\circ} \, 2 \, \textbf{cm}$  & $5^{\circ} \, 5 \, \textbf{cm}$  & $10^{\circ} \, 2 \, \textbf{cm}$ & $10^{\circ} \, 5 \, \textbf{cm}$ & $IoU_{50}$ & \multicolumn{1}{c|}{$IoU_{75}$} & $5^{\circ} \, 2 \, \textbf{cm}$  & $5^{\circ} \, 5 \, \textbf{cm}$  & $10^{\circ} \, 2 \, \textbf{cm}$ & $10^{\circ} \, 5 \, \textbf{cm}$ \\ \hline
    bottle                    & 93.7  & \multicolumn{1}{c|}{91.4}  & 80.9 & 96.4 & 82.3 & 99   & 57.7  & \multicolumn{1}{c|}{50.3}  & 62   & 64.9 & 83.4 & 88   \\
    bowl                      & 96.9  & \multicolumn{1}{c|}{96.7}  & 98.7 & 99   & 99.7 & 99.8 & 100   & \multicolumn{1}{c|}{100}   & 88.7 & 94.3 & 94.1 & 99.7 \\
    camera                    & 89.2  & \multicolumn{1}{c|}{84.3}  & 57   & 60.9 & 73.6 & 81.1 & 90.8  & \multicolumn{1}{c|}{82.9}  & 1.2  & 1.3  & 24.8 & 27.3 \\
    can                       & 92.1  & \multicolumn{1}{c|}{92}    & 99.7 & 99.8 & 99.7 & 99.9 & 71.3  & \multicolumn{1}{c|}{71.2}  & 83.4 & 85.3 & 96.3 & 98.6 \\
    laptop                    & 97.5  & \multicolumn{1}{c|}{90.8}  & 76.1 & 85.9 & 80.6 & 92.4 & 83.3  & \multicolumn{1}{c|}{74.1}  & 59.6 & 91.1 & 61.2 & 95.6 \\
    mug                       & 93.6  & \multicolumn{1}{c|}{92.7}  & 54.5 & 54.6 & 77.1 & 77.3 & 99.4  & \multicolumn{1}{c|}{98.5}  & 32.9 & 33.4 & 88.3 & 89.3 \\ \hline
    average                   & 93.8  & \multicolumn{1}{c|}{91.3}  & 77.8 & 82.8 & 85.5 & 91.6 & 83.7  & \multicolumn{1}{c|}{79.5}  & 54.7 & 61.7 & 74.7 & 83.1 \\ \hline
    \end{tabular}
\end{table*}

==> cvpr2024/table/real_per_cat.tex <==
\begin{table}[h]
    \setlength{\tabcolsep}{3pt}
    \caption{\textbf{
        Per-category results of AG-Pose on REAL275.}
        }
    \label{tab:REAL275_per_cat}
    \centering
    \begin{tabular}{c|cc|cccc}
        \hline
        category & $IoU_{50}$ & $IoU_{75}$ & $5^{\circ} \, 2 \, \textbf{cm}$  & $5^{\circ} \, 5 \, \textbf{cm}$  & $10^{\circ} \, 2 \, \textbf{cm}$ & $10^{\circ} \, 5 \, \textbf{cm}$ \\ \hline
        bottle   & 57.7  & 50.3  & 62   & 64.9 & 83.4 & 88   \\
        bowl     & 100   & 100   & 88.7 & 94.3 & 94.1 & 99.7 \\
        camera   & 90.8  & 82.9  & 1.2  & 1.3  & 24.8 & 27.3 \\
        can      & 71.3  & 71.2  & 83.4 & 85.3 & 96.3 & 98.6 \\
        laptop   & 83.3  & 74.1  & 59.6 & 91.1 & 61.2 & 95.6 \\
        mug      & 99.4  & 98.5  & 32.9 & 33.4 & 88.3 & 89.3 \\ \hline
        average  & 83.7  & 79.5  & 54.7 & 61.7 & 74.7 & 83.1 \\ \hline
        \end{tabular}
    \end{table}
